Unleashing Low-Bit Inference on Ascend NPUs: A Comprehensive Evaluation of HiFloat Formats

As LLMs scale, low-bit floating-point formats like MXFP and NVFP4 offer new opportunities for precision and efficiency. In this work, we evaluate HiFloat (HiF8 and HiF4), a family of formats tailored for Ascend NPUs. Through rigorous comparison across weight-activation and KV-cache tasks, we provide three key insights: (1) INT8 suits narrow-range data, while floating-point formats excel with high-variance data; (2) in 4-bit regimes, HiF4's hierarchical scaling prevents the accuracy collapse seen in integer formats; and (3) HiFloat is fully compatible with state-of-the-art post-training quantization frameworks. Overall, HiFloat provides a solution for high-efficiency LLM inference on NPUs.

==> doc/quant_method.tex <==
\section{PTQ Integration for HiFloat} \label{sec:quant}
While our previous analysis focused on the intrinsic fidelity of the HiFloat formats, the deployment of LLMs often necessitates advanced PTQ methods to further minimize accuracy degradation. In this section, we investigate the integration of HiF8 and HiF4 with established PTQ techniques, specifically SmoothQuant~\citep{xiao2023smoothquant} and SVDQuant~\citep{li2024svdquant}, and compare their performance against other formats. Although these methods were originally designed to mitigate the limitations of integer quantization, we evaluate their efficacy in the floating-point domain to determine if they can further narrow the gap to original performance.


\subsection{SmoothQuant} \label{sec:smoothquant}
As stated by our fidelity results in Sections~\ref{sec:hif8} and~\ref{sec:hif4}, quantizing LLMs faces a fundamental asymmetric challenge: while weights exhibit relatively uniform distributions, activations are plagued by channel-wise persistent outliers that significantly inflate quantization error. To resolve this, SmoothQuant~\citep{xiao2023smoothquant} introduces a mathematically equivalent transformation that migrates the quantization difficulty from the activations to the weights. By scaling down activation spikes and correspondingly scaling up the weights, the method balances the precision requirements of both tensors, making them more amenable to low-bit formats without sacrificing accuracy. Specifically, for a linear layer $\mathbf{Y} = \mathbf{X}\mathbf{W}$, SmoothQuant achieves this via a per-channel scaling transformation $\mathbf{s}$:
\begin{equation}\label{equ:smoothquant}
    \mathbf{Y} = (\mathbf{X} \text{diag}(\mathbf{s})^{-1}) \cdot (\text{diag}(\mathbf{s}) \mathbf{W}),
\end{equation}
where the smoothing factor $s_j$ for the $j$-th channel is derived from the maximum values of activations and weights:
\begin{equation}
    s_j = \max(|\mathbf{X}_{:,j}|)^\alpha / \max(|\mathbf{W}_{j,:}|)^{1-\alpha},
\end{equation}
where the hyperparameter $\alpha$ controls the migration strength.

The original SmoothQuant study demonstrated significant accuracy improvements for W8A8 integer quantization. This aligns with our fidelity results in Figures~\ref{fig:sqnr_8bit_w} and~\ref{fig:sqnr_8bit_a}, which show that while INT8 maintains high fidelity for weight quantization, it suffers significantly when applied to activations due to the presence of outliers. Based on our fidelity rankings, the efficacy of SmoothQuant across 8-bit formats is determined by their capacity to absorb weight-side variance. While INT8 and MXFP8 possess the high weight SQNR necessary to provide a fidelity budget for migrated outliers, formats like E5M2 and HiF8 reside at the bottom of the weight fidelity hierarchy, making them more sensitive to the increased weight range induced by the smoothing transformation. Consequently, while SmoothQuant effectively addresses the activation-side bottleneck for INT8, its application to HiF8 requires a finer balance to ensure that the gains in activation precision are not offset by a collapse in weight-side reconstruction.

In the W4A4 quantization regime, the fidelity budget for SmoothQuant shifts significantly. Our results show that HiF4 maintains the highest weight fidelity, providing a superior foundation for absorbing migrated activation outliers compared to NVFP4 or MXFP4. Interestingly, while NVFP4 and HiF4 exhibit comparable activation fidelity, HiF4’s lead in weight SQNR suggests it can tolerate more aggressive smoothing without the weight-side collapse that limits other 4-bit formats. This indicates that the hierarchical scaling of HiF4 is uniquely suited to the W4A4 challenge. As for INT4, the limited performance of its weight quantization means that the cost of migrating outliers often outweighs the benefits; the resulting distortion in the weights can be as damaging as the original activation outliers, preventing SmoothQuant from delivering a fundamental accuracy improvement.

% \subsubsection{Algorithm Overview}

% SmoothQuant exploits the mathematical equivalence of linear layer computation under per-channel scaling. For a linear layer $Y = XW$ with input $X \in \mathbb{R}^{b \times m}$ and weight $W \in \mathbb{R}^{m \times n}$, we introduce a diagonal scaling matrix:
% \begin{equation}
% Y = XW = (X \cdot \text{diag}(s)^{-1}) \cdot (\text{diag}(s) \cdot W) = \hat{X} \hat{W}
% \end{equation}
% where $s \in \mathbb{R}^m$ is a per-channel smoothing factor, $\hat{X} = X \cdot \text{diag}(s)^{-1}$ is the smoothed activation, and $\hat{W} = \text{diag}(s) \cdot W$ is the adjusted weight. The smoothing factor $s$ is computed to balance the quantization difficulty between activations and weights, $s_j = \frac{\max(|X_{:,j}|)^\alpha}{\max(|W_{j,:}|)^{1-\alpha}}$, where $\alpha \in [0, 1]$ is a migration strength hyperparameter. When $\alpha = 1$, all difficulty remains in activations; when $\alpha = 0$, all difficulty migrates to weights; typical values of $\alpha \in [0.5, 0.75]$ achieve balanced quantization error. The quantized computation becomes:
% \begin{equation}
% Y \approx Q(\hat{X}) \cdot Q(\hat{W}) = Q(X \cdot \text{diag}(s)^{-1}) \cdot Q(\text{diag}(s) \cdot W)
% \end{equation}

% \subsubsection{Effectiveness and Limitations}

% SmoothQuant's effectiveness stems from two properties:

% \begin{itemize}
%     \item Offline integration: The scaling factor $s$ can be fused into preceding LayerNorm weights or biases, adding zero runtime overhead.
%     \item Channel-wise migration: By scaling down outlier channels in activations and correspondingly scaling up weights, both tensors achieve more uniform magnitude distributions.
% \end{itemize}

% However, SmoothQuant has inherent limitations for aggressive quantization:

% \begin{itemize}
%     \item Zero-sum redistribution: Outliers are relocated, not eliminated. Reducing activation range necessarily increases weight range, limiting benefits when both sides are quantization-sensitive.
%     \item Diminishing returns at 4-bit: At W8A8, the redistribution achieves near-lossless quantization. At W4A4, both sides become highly sensitive, and no $\alpha$ value can simultaneously satisfy both constraints.
%     \item Per-tensor scaling assumption: SmoothQuant assumes per-tensor or per-channel quantization; it does not exploit finer-grained block-wise scaling available in modern formats.
% \end{itemize}


% \subsubsection{Analysis on SmoothQuant with HiFloat}

% \paragraph{SmoothQuant with HiF8}
% HiF8's extended 38-binade dynamic range significantly reduces the need for smoothing:

% \begin{itemize}
%     \item Reduced clipping: Activation outliers that would clip in E4M3/E5M2 remain representable in HiF8's tapered regions, even without smoothing.
%     \item Complementary benefits: SmoothQuant can still provide marginal improvements by concentrating values in HiF8's high-precision central region rather than the reduced-precision tails, although the $\alpha$ hyperparameter becomes less critical since HiF8 tolerates wider ranges on both sides. 
% \end{itemize}

% For HiF8 deployment, SmoothQuant remains beneficial but is no longer essential---the format's native dynamic range handles most outlier scenarios that would otherwise require careful $\alpha$ tuning.

% \paragraph{SmoothQuant with HiF4}
% The interaction with HiF4 is more nuanced due to HiF4's hierarchical block-wise scaling:

% \begin{table}[h]
% \centering
% \caption{SmoothQuant Interaction with HiF4 Hierarchical Scaling}
% \label{tab:smoothquant_HiF4}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc}
% \toprule
% Aspect & SmoothQuant Effect & HiF4 Synergy \\
% \midrule
% Cross-channel outliers & Redistributed to weights & Reduces $S_1$ variance \\
% Intra-block variance & Unchanged & Handled by $E_2$, $E_3$ \\
% Weight magnitude increase & Increases $\|\hat{W}\|$ & May increase $S_1$ range \\
% Offline overhead & Zero (fused into LayerNorm) & Compatible \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% The combined approach proceeds as: $Y \approx Q_{\text{HiF4}}(\hat{X}) \cdot Q_{\text{HiF4}}(\hat{W})$. Key observations for this combination:
% \begin{itemize}
%     \item Reduced block scale variance: Smoothed activations $\hat{X}$ exhibit more uniform per-block magnitudes, reducing the range that each $S_1$ scale must cover.
%     \item Preserved intra-block adaptation: HiF4's $E_2$ and $E_3$ refinements continue to handle within-block variations that SmoothQuant does not address.
%     \item Weight-side trade-off: The increased weight magnitudes in $\hat{W}$ may require larger $S_1$ scales for weight blocks, partially offsetting activation-side improvements.
% \end{itemize}

% \subsubsection{Comparison: SmoothQuant vs. HiF4 Native Scaling}

% A practical question is whether SmoothQuant provides meaningful benefits when HiF4's hierarchical scaling already adapts to local magnitude variations:

% \begin{table}[h]
% \centering
% \caption{Outlier Handling: SmoothQuant vs. HiF4 Hierarchical Scaling}
% \label{tab:smooth_vs_HiF4}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc}
% \toprule
% Outlier Type & SmoothQuant Handling & HiF4 Native Handling \\
% \midrule
% Channel-wise persistent & Migrated to weights & Per-block $S_1$ adaptation \\
% Token-wise transient & Not addressed & $E_2$, $E_3$ refinement \\
% Global magnitude shift & Balanced via $\alpha$ & Block-independent scaling \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% Empirically, the benefit of SmoothQuant with HiF4 depends on the outlier structure:
% \begin{itemize}
%     \item For models with \textbf{strong channel-wise outliers} (e.g., OPT, BLOOM), SmoothQuant preprocessing improves HiF4 quantization by reducing cross-block scale variance.
%     \item For models with \textbf{distributed outliers} (e.g., LLaMA, Mistral), HiF4's native hierarchical scaling suffices, and SmoothQuant provides marginal additional benefit.
%     \item For \textbf{W4A4 quantization}, SmoothQuant alone is insufficient regardless of format, where the redistributed outliers still challenge 4-bit weights, motivating SVDQuant's absorption approach.
% \end{itemize}


%======================
\subsection{SVDQuant}
SVDQuant~\citep{li2024svdquant} addresses the outlier challenge by decoupling the weight matrix into a low-bit base component and a high-precision low-rank branch. Recognizing that activation outliers often manifest in specific directions of the feature space, SVDQuant employs Singular Value Decomposition (SVD) to identify and extract the most salient outliers into a separate, low-rank product. Specifically, for a weight matrix $\mathbf{W}$, SVDQuant decompose it as follows:
\begin{equation}
    \mathbf{W} \approx \hat{\mathbf{W}} + \mathbf{L}_1\mathbf{L}_2,
\end{equation}
where $\hat{\mathbf{W}}$ is the quantized residual matrix and $\mathbf{L}_1\mathbf{L}_2$ represents the low-rank approximation of the outliers. The SVDQuant pipeline generally incorporates an initial smoothing step, analogous to SmoothQuant shown in Equation~\ref{equ:smoothquant}, before performing the low-rank decomposition.

While SVDQuant absorbs structurally salient components, specifically those represented by the largest singular values, into a high-precision branch, the remaining residual matrix presents a distinct numerical challenge. This residual does not necessarily follow a distribution that is naturally compatible with standard data formats. Furthermore, because SVDQuant is typically executed as a refinement of the SmoothQuant transformation, its overall efficacy remains fundamentally bounded by the quality of the initial scaling step. This suggests that a format capable of adaptive local precision is required to accurately capture the nuanced structure that remains after the primary singular components are removed.

% While HiFloat formats provide improved dynamic range (HiF8) and intra-block adaptation (HiF4), extreme outliers in weights and activations can still challenge 4-bit quantization~\citep{he2025preserving}. This section examines SVDQuant~\citep{li2024svdquant}, a complementary technique that absorbs outliers through low-rank decomposition, and analyzes its interaction with HiFloat formats.

% \subsubsection{Motivation: Limitations of Outlier Redistribution}

% Traditional outlier mitigation techniques like SmoothQuant~\citep{xiao2023smoothquant} redistribute outliers between activations and weights using per-channel scaling factors. Given input $X \in \mathbb{R}^{b \times m}$ and weight $W \in \mathbb{R}^{m \times n}$, smoothing transforms:
% \begin{equation}
% XW = \underbrace{(X \cdot \text{diag}(\lambda)^{-1})}_{\hat{X}} \cdot \underbrace{(\text{diag}(\lambda) \cdot W)}_{\hat{W}}
% \end{equation}
% where $\lambda \in \mathbb{R}^m$ is a per-channel scaling factor.

% While this reduces activation outliers in $\hat{X}$, it amplifies weight outliers in $\hat{W}$. For W4A4 quantization where both sides are highly sensitive, this redistribution provides limited benefit---the outliers are merely relocated, not eliminated. SVDQuant addresses this limitation by introducing a high-precision low-rank branch to \emph{absorb} rather than redistribute outliers. The key insight is that after smoothing, the weight matrix $\hat{W}$ exhibits a sharply decaying singular value spectrum, with outliers concentrated in the top few singular values.

% \subsubsection{Algorithm Overview}

% The method proceeds in two stages:
% (1) Outlier Consolidation. First, migrate outliers from activations to weights via smoothing, producing $\hat{X}$ (low outliers) and $\hat{W}$ (concentrated outliers).
% (2) Low-Rank Decomposition. Decompose the smoothed weight using truncated SVD:
% \begin{equation}
% \hat{W} = U\Sigma V^\top \approx \underbrace{U_{:,:r} \Sigma_{:r,:r} V_{:r,:}^\top}_{L_1 L_2} + \underbrace{(\hat{W} - L_1 L_2)}_{R}
% \end{equation}
% where $r \ll \min(m, n)$ is the rank (typically 16--32), $L_1 = U_{:,:r} \Sigma_{:r,:r}^{1/2} \in \mathbb{R}^{m \times r}$, and $L_2 = \Sigma_{:r,:r}^{1/2} V_{:r,:}^\top \in \mathbb{R}^{r \times n}$.
% The linear layer computation becomes:
% \begin{equation}
% XW = \hat{X}\hat{W} \approx \underbrace{\hat{X} L_1 L_2}_{\text{16-bit low-rank branch}} + \underbrace{Q(\hat{X}) Q(R)}_{\text{4-bit quantized branch}}
% \label{eq:svdquant_decomp}
% \end{equation}

% The effectiveness stems from two properties: \textit{Outlier Concentration}: After smoothing, the singular value distribution of $\hat{W}$ becomes highly imbalanced, with the first few singular values dominating. Removing these via the low-rank branch dramatically reduces the magnitude and outlier content of the residual $R$. \textit{Quantization Error Bound}: For residual $R$ with reduced magnitude, the quantization error is bounded by:
%     \begin{equation}
%     \mathbb{E}[\|R - Q(R)\|_F] \leq \frac{c\sqrt{\text{size}(R)}}{q_{\max}} \cdot \mathbb{E}[\|R\|_F]
%     \end{equation}
%     where $\|R\|_F = \sqrt{\sum_{i=r+1}^{\min(m,n)} \sigma_i^2}$ is significantly smaller than $\|\hat{W}\|_F$ after removing the top-$r$ singular values.


% \subsubsection{Analysis on SVDQuant with HiFloat}

% \paragraph{SVDQuant with HiF8} 

% The interaction between SVDQuant and HiF8 reveals an interesting trade-off between algorithmic and format-level outlier handling. HiF8's 38-binade dynamic range provides substantial native outlier tolerance through its tapered precision design—values that would overflow in E4M3 or E5M2 remain representable in HiF8, albeit with gracefully degraded precision in the extended exponent regions.

% This native capability reduces, but does not eliminate, the benefits of SVDQuant:

% \begin{itemize}
%     \item \textbf{Reduced clipping necessity}: HiF8's extended range accommodates magnitude outliers without the hard clipping that motivates SVDQuant for narrower formats. Per-tensor scaling often suffices, as HiF8's design inherently assumes this scaling granularity.
    
%     \item \textbf{Precision recovery for extreme outliers}: While HiF8 \textit{represents} outliers, it does so with reduced mantissa precision (1-2 bits in the extended regions). For tensors where outlier channels carry critical information—such as attention output projections in certain architectures—SVDQuant's low-rank branch preserves these values at full BF16 precision, potentially improving task-specific accuracy.
    
%     \item \textbf{Complementary coverage}: SVDQuant absorbs \textit{structured} outliers (low-rank patterns), while HiF8 handles \textit{unstructured} magnitude variations. When both outlier types coexist, the combination provides comprehensive coverage.
% \end{itemize}

% Our empirical results (Table~\ref{tab:svdquant_results}) indicate that SVDQuant provides marginal but consistent improvements for HiF8 quantization, with perplexity reductions of 0.1--0.3 points on Qwen3-8B. The improvement is more pronounced for models with known outlier channels (e.g., LLaMA-family architectures) compared to models with smoother activation distributions.

% \paragraph{SVDQuant with HiF4}

% The interaction between SVDQuant and HiF4 is more nuanced, as both mechanisms address outlier handling through fundamentally different approaches. HiF4's hierarchical scaling ($S_1$, $E_2$, $E_3$) provides \textit{local} adaptation within and across blocks, while SVDQuant's low-rank decomposition captures \textit{global} structural patterns. Understanding their complementarity requires analyzing different outlier types:

% \begin{table}[h]
% \centering
% \caption{Outlier Handling Mechanisms: HiF4 vs. SVDQuant}
% \label{tab:svdquant_HiF4}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% \textbf{Outlier Type} & \textbf{Spatial Pattern} & \textbf{HiF4 Handling} & \textbf{SVDQuant Benefit} \\
% \midrule
% Intra-block magnitude & Within 64 elements & $E_2$, $E_3$ sub-block adaptation & Limited \\
% Cross-block magnitude & Between blocks & $S_1$ (E6M2) per-block scaling & Moderate \\
% Channel-wise structured & Consistent across tokens & Block-independent & Significant \\
% Low-rank patterns & Global correlation & Not addressed & Significant \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% This analysis motivates a combined approach where SVDQuant preprocessing enhances HiF4's effectiveness. Following the decomposition $W = L_1 L_2 + R$, we quantize only the residual:
% \begin{equation}
%     XW \approx X L_1 L_2 + Q_{\text{HiF4}}(X) \cdot Q_{\text{HiF4}}(R),
% \end{equation}
% where the low-rank component $L_1 L_2$ is computed at full precision (or higher-precision quantization), and the residual $R$ undergoes HiF4 quantization.

% The key insight is that SVDQuant's low-rank extraction \textit{conditions} the residual distribution for more effective HiF4 quantization:

% \begin{itemize}
%     \item \textbf{Compressed dynamic range}: After removing dominant singular components, the residual $R$ exhibits reduced magnitude variation. This allows HiF4's E6M2 block scale $S_1$ to operate over a narrower range, reducing scale quantization error.
    
%     \item \textbf{Reduced hierarchical refinement}: With a more uniform residual distribution, fewer sub-blocks require the $E_2 = 1$ or $E_3 = 1$ extended-range refinements. This effectively increases the average mantissa precision across the tensor.
    
%     \item \textbf{Better grid utilization}: The E0M3 element grid, which provides uniform 3-bit mantissa precision within each sub-block's adapted range, better matches the compressed residual distribution compared to the original weight distribution.
% \end{itemize}

% \paragraph{Comparison with Alternative Approaches}

% A natural question arises: can HiF4's native hierarchical scaling achieve comparable outlier handling to MXFP4 combined with SVDQuant? Table~\ref{tab:HiF4_vs_mxfp4_svd} summarizes the trade-offs:

% \begin{table}[h]
% \centering
% \caption{Native Hierarchical Scaling vs. Low-Rank Decomposition}
% \label{tab:HiF4_vs_mxfp4_svd}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcc}
% \toprule
% \textbf{Aspect} & \textbf{HiF4 (native)} & \textbf{MXFP4 + SVDQuant} \\
% \midrule
% Intra-block adaptation & $4\times$ range via $E_2$, $E_3$ & Single shared scale \\
% Cross-block handling & Independent $S_1$ per block & Low-rank branch absorption \\
% Effective bits/element & 4.5 (including scales) & 4.0 + $\sim$0.26 (rank-64) \\
% Inference overhead & Hierarchical dequantization & Additional low-rank matmul \\
% Calibration requirement & Block-wise statistics & SVD + scale calibration \\
% Outlier specificity & Magnitude-based & Structure-aware \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% The choice between these approaches depends on the dominant outlier characteristics of the target model:

% \begin{itemize}
%     \item \textbf{Local magnitude outliers}: When outliers arise from activation-dependent scaling or sporadic large values without consistent spatial structure, HiF4's hierarchical scaling provides efficient, automatic adaptation without additional calibration complexity. The sub-block refinements ($E_2$, $E_3$) dynamically adjust to local magnitude variations during dequantization.
    
%     \item \textbf{Global structured outliers}: When outliers exhibit low-rank structure—such as consistent outlier channels across token positions or correlated activation patterns—SVDQuant more effectively absorbs these patterns into the full-precision low-rank branch. MXFP4's simpler per-block scaling then suffices for the well-conditioned residual.
    
%     \item \textbf{Mixed outlier patterns}: For models exhibiting both local and global outliers, the combination of SVDQuant with HiF4 provides comprehensive coverage: low-rank decomposition handles structured patterns, while hierarchical scaling adapts to residual magnitude variations.
% \end{itemize}

% \paragraph{Practical Recommendations}

% Based on our analysis and empirical observations, we provide the following guidelines for SVDQuant integration with HiFloat formats:

% \begin{enumerate}
%     \item \textbf{HiF8 quantization}: SVDQuant is optional. Apply when targeting models with known extreme outlier channels or when pursuing the highest possible accuracy. The overhead-to-benefit ratio is less favorable compared to narrower formats.
    
%     \item \textbf{HiF4 quantization}: SVDQuant is recommended. The 4-bit precision constraint amplifies the impact of outliers; low-rank preprocessing consistently improves quantization quality. Use rank-32 to rank-64 for optimal overhead-accuracy trade-off.
    
%     \item \textbf{Mixed-precision deployment}: Consider HiF8 for attention layers (which exhibit more dynamic activation patterns) and HiF4 with SVDQuant for FFN layers (which benefit more from low-rank decomposition due to their structured weight matrices).
% \end{enumerate}


%============================
% \subsection{KV Cache and Attention Quantization}



% The Key-Value (KV) cache represents a critical memory bottleneck in auto-regressive LLM inference~\citep{KIVI, hooper2025kvquant, li2025kvtuner}. KV cache grows linearly with sequence length and batch size, often dominating memory consumption for long-context applications during the decoding phase. Unlike weight-activation quantization, which can be performed offline with extensive calibration for optimized quantization scales, KV cache quantization normally operates \textit{online} during inference, imposing stringent constraints on computational overhead and robustness to distribution drift during online generation.

% \subsubsection{Challenges in KV Cache Quantization}

% KV cache quantization presents unique challenges distinct from weight and activation quantization:

% \begin{itemize}
%     \item \textbf{Online Quantization Requirement}: KV states are generated dynamically during inference, precluding the use of calibration-based methods. The offline calibrated static KV cache quantization cannot well fit the diverse data distributions.
    
%     \item \textbf{Heterogeneous Value Distributions}: KV cache values exhibit substantial variation across attention heads, layers, and token positions. Early tokens (e.g., attention sinks) often display different magnitude characteristics compared to later tokens, posing challenges for per-tensor quantization granularity.
    
%     \item \textbf{Asymmetric Sensitivity}: Prior work~\cite{li2025kvtuner} has demonstrated that Key and Value states exhibit different quantization sensitivities. Key states, which determine attention patterns through dot-product similarity, are generally more sensitive to quantization noise than Value states, which serve as weighted aggregation targets.
    
%     \item \textbf{Accumulating Error}: KV cache quantization directly results in attention distribution shift. Quantization errors in early tokens propagate through attention computations in subsequent layers and steps, potentially amplifying errors over long sequences.
% \end{itemize}


% \subsubsection{Quantization Strategies for KV Cache}
% We consider two primary quantization strategies for KV cache compression:

% \textbf{Per-Token Quantization.} The straightforward approach applies independent quantization to each token's KV representation:
% \begin{equation}
%     \mathbf{K}_t^q = Q(\mathbf{K}_t), \quad \mathbf{V}_t^q = Q(\mathbf{V}_t),
% \end{equation}
% where $Q(\cdot)$ denotes the quantization operator and $t$ indexes the token position. This strategy is naturally compatible with autoregressive generation but fails to exploit cross-token redundancy.

% % \textbf{Per-Channel Quantization.} Motivated by the observation that certain channels consistently exhibit larger magnitudes, per-channel quantization computes scaling factors across the token dimension:
% % \begin{equation}
% %     s_c = \max_{t} |\mathbf{K}_{t,c}|, \quad \mathbf{K}^q_{:,c} = Q(\mathbf{K}_{:,c} / s_c),
% % \end{equation}
% % where $c$ indexes the channel dimension. This approach better accommodates channel-wise outliers but requires maintaining per-channel statistics during generation.

% \textbf{Block-wise Quantization.} For formats supporting block-wise scaling (MXFP, NVFP, HiF4), KV states are partitioned into micro-blocks with shared scaling factors:
% \begin{equation}
%     \mathbf{K}^q_{[b]} = s_{[b]} \cdot Q_E(\mathbf{K}_{[b]} / s_{[b]}),
% \end{equation}
% where $[b]$ denotes the block index and $Q_E(\cdot)$ quantizes to the element data type. This strategy naturally adapts to local magnitude variations without explicit outlier handling.

% \subsubsection{Analysis on KV Cache Quantization with HiFloat}
% Table~\ref{tab:kv-comparison} summarizes the trade-offs between formats for KV cache quantization.
% \begin{table}[h]
% \centering
% \caption{Format Comparison for KV Cache Quantization}
% \label{tab:kv-comparison}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|ccc}
% \toprule
% \textbf{Property} & \textbf{INT4/8} & \textbf{MXFP4/8} & \textbf{HiF4/8} \\
% \midrule
% Online quantization & Global & Block-local & Block-local \\
% Outlier tolerance & Poor & Moderate & High \\
% Cross-head adaptation & Per-head scaling & Per-block & Hierarchical \\
% Dequantization cost & Minimal & Low & Moderate \\
% Ascend NPU support & Partial & Limited & Native \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \textbf{HiF8 for KV Cache.} HiF8's extended dynamic range (38 binades) provides significant advantages for online KV cache quantization than the INT8 data format:

% \begin{itemize}
%     \item \textbf{Robustness to Distribution Drift}: The variable-mantissa design automatically allocates precision based on magnitude. Attention sink tokens with atypical magnitudes are accommodated without clipping, while typical tokens benefit from high precision in the central range.
    
%     \item \textbf{Simplified Scaling}: Unlike INT8, which requires careful per-channel or per-token scale calibration, HiF8's inherent dynamic range often permits per-tensor scaling without significant accuracy loss, reducing the metadata overhead.
% \end{itemize}

% However, as our SQNR analysis in Figure \ref{fig:layer_wise_sqnr_qwen3_8b_8bit_format} reveals, HiF8 does not uniformly outperform alternatives for KV cache. For Value states with relatively bounded distributions, the simpler MXFP8 format achieves comparable or superior SQNR due to its consistent 4-bit mantissa precision within the active range.

% \textbf{HiF4 for KV Cache.} As demonstrated in Figure \ref{fig:layer_wise_sqnr_qwen3_8b_4bit_format}, the three-stage hierarchical scaling structure of HiF4 is particularly well-suited for KV cache quantization:

% \begin{itemize}
%     \item \textbf{Intra-block Adaptation}: A single 64-element KV macro-block may span multiple token positions with varying scales in different channels. HiF4's sub-block refinements ($E_2$, $E_3$) provide up to $4\times$ intra-block dynamic range adjustment, automatically accommodating this heterogeneity. The HiF4 fine-grained hierarchical scaling also leaves more space for channel-reordering to improve data spatial locality than the global scale of NVFP4.
    
%     % \item \textbf{Cross-head Robustness}: Different attention heads often operate at different magnitude scales. HiF4's per-block $S_1$ scaling (E6M2) independently adapts to each head's distribution .
    
%     \item \textbf{Online Efficiency}: Despite its hierarchical structure, HiF4 quantization requires only local maximum computations within each block, maintaining $O(1)$ complexity per element suitable for online deployment.
% \end{itemize}


% \subsubsection{Asymmetric Key-Value Quantization}

% Given the differential sensitivity of Key and Value states, we investigate asymmetric precision allocation. Specifically, we consider configurations where Key states are quantized at higher precision than Value states (K8V4) or vice versa (K4V8).

% The rationale for asymmetric quantization stems from their distinct roles in attention computation:
% \begin{equation}
%     \text{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}\left(\frac{\mathbf{Q}\mathbf{K}^\top}{\sqrt{d_k}}\right) \mathbf{V}.
% \end{equation}

% Key states influence attention weight computation through dot-product similarity with queries. Quantization errors in $\mathbf{K}$ directly perturb the attention distribution, potentially redirecting attention to incorrect tokens. In contrast, Value states serve as the aggregation targets; quantization errors in $\mathbf{V}$ manifest as additive noise in the output, which may be partially averaged out through the weighted sum.

% For HiFloat formats, we observe that:
% \begin{itemize}
%     \item \textbf{K8V4 Configuration}: Preserving Key precision with HiF8 while aggressively quantizing Values with HiF4 maintains attention pattern fidelity. HiF4's hierarchical scaling compensates for Value magnitude variations across heads.
    
%     \item \textbf{K4V8 Configuration}: This allocation is generally suboptimal, as 4-bit Key quantization introduces attention distribution errors that 8-bit Value precision cannot recover.
% \end{itemize}

% Our experimental results (Table~\ref{tab:kv-results}) validate these observations, demonstrating that appropriate format selection and precision allocation can achieve substantial memory reduction with minimal perplexity degradation.

% \subsubsection{Integration with Weight-Activation Quantization}

% A practical deployment scenario involves simultaneous quantization of weights, activations, and KV cache. We investigate the interaction effects when combining HiFloat KV cache and attention quantization with weight-activation quantization methods (SmoothQuant, SVDQuant).

% Key observations from our experiments:
% \begin{itemize}
%     \item \textbf{Error Accumulation}: When weights and activations are quantized to W4A4, additional KV cache quantization amplifies errors non-linearly. The choice of KV format becomes critical—HiF4's robustness provides a larger error budget compared to MXFP4 and NVFP4.
    
%     \item \textbf{Format Consistency}: Using consistent formats across weights, activations, and KV cache (e.g., all HiFloat or all MXFP) simplifies hardware implementation and often yields comparable or better results than mixed-format configurations.
    
%     \item \textbf{Attention Quantization}: Beyond KV cache, quantizing the attention computation itself ($\mathbf{Q}\mathbf{K}^\top$ and softmax-weighted aggregation) introduces additional error sources. HiF8's extended range proves beneficial for representing the pre-softmax logits than INT8, which can span several orders of magnitude.
% \end{itemize}

% Thus, HiFloat formats offer compelling advantages for KV cache and attention quantization, particularly in online scenarios where calibration is impractical and distribution heterogeneity is unavoidable. The hierarchical scaling of HiF4 and extended dynamic range of HiF8 provide native outlier tolerance that reduces the need for sophisticated preprocessing techniques required by integer formats.



% \subsubsection{Overhead Considerations}

% The low-rank branch adds $\frac{mr + nr}{mn} = \frac{r(m+n)}{mn}$ relative overhead in parameters and computation. For typical dimensions ($m, n \approx 4096$) and $r = 32$, this is approximately 1.6\%. However, naively executing the low-rank branch as separate kernels incurs significant memory access overhead ($\sim$50\% latency increase) due to activation data movement. The Nunchaku inference engine addresses this through kernel fusion: the down-projection $L_1$ shares input with the quantization kernel, while the up-projection $L_2$ shares output with the 4-bit computation kernel, reducing the overhead to 5-10\%.

% Based on the analysis:

% \begin{enumerate}
%     \item \textbf{HiF8 deployment}: SVDQuant provides marginal benefits; the native format's extended range is usually sufficient for inference scenarios.
    
%     \item \textbf{HiF4 for weights}: Consider SVDQuant for layers with known global outlier patterns (e.g., attention QKV projections). The low-rank branch overhead is acceptable for weight-heavy inference.
    
%     \item \textbf{HiF4 for activations}: SVDQuant is less applicable since activations are quantized online. HiF4's hierarchical scaling handles dynamic outliers more naturally.
    
%     \item \textbf{Hybrid approach}: For maximum quality, use SVDQuant on weights and rely on HiF4's native hierarchical scaling for activations. This combines the strengths of both approaches.
% \end{enumerate}
